Contrastive Representation Distillation

Often we wish to transfer representational knowledge from one neural network to another. Examples include distilling a large network into a smaller one, transferring knowledge from one sensory modality to a second, or ensembling a collection of models into a single estimator. Knowledge distillation, the standard approach to these problems, minimizes the KL divergence between the probabilistic outputs of a teacher and student network. We demonstrate that this objective ignores important structural knowledge of the teacher network. This motivates an alternative objective by which we train a student to capture significantly more information in the teacher's representation of the data. We formulate this objective as contrastive learning. Experiments demonstrate that our resulting new objective outperforms knowledge distillation and other cutting-edge distillers on a variety of knowledge transfer tasks, including single model compression, ensemble distillation, and cross-modal transfer. Our method sets a new state-of-the-art in many transfer tasks, and sometimes even outperforms the teacher network when combined with knowledge distillation. Code: http://github.com/HobbitLong/RepDistiller.

==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> text/method_nce.tex <==
\subsection{NCE approximation}
\vspace{-5pt}

The contrastive loss is most effective with a large number of negative samples. Computing the full softmax contrastive loss Eq. \ref{eqn:contrastive_loss} is prohibitively expensive for large scale datasets such as Imagenet \cite{deng2009imagenet}. Similar to recent works~\cite{mnih2013learning,wu2018unsupervised,mnih2013learning}, we approximate the full softmax by resorting to Noise Contrastive Estimation \cite{gutmann2010noise} (NCE), which is a method to estimate parameters of unnormalized statistical models. The basic idea is learning to differentiate observed data from auxiliary noise by logistic regression. We first rewrite Eq.~\ref{eqn:contrastive_loss} in a probabilistic format. Given $x_i$, for any sample $x$, the probability that the feature $f^S(x)$ produced by the student network matches the feature $f^T(x_i)$ from the teacher network is:

\vspace{-10pt}

\begin{eqnarray}
    p(x|x_i;f^T,f^S)=\frac{\exp(f^T(x_i)^{\prime} f^S(x)/ \tau)}{\sum_{j=1}^N \exp(f^T(x_j)^{\prime} f^S(x)/\tau)}
    \label{eqn:prob}
    \vspace{-5pt}
\end{eqnarray}

where $\tau$ is a temperature that modifies the distribution and $Z = \sum_{j=1}^N \exp(f^T(x_j)^{\prime} f^S(x)/\tau)$ is the normalization factor, which is expensive to compute. Eq.~\ref{eqn:contrastive_loss} is equivalent to $\mathbb{E}[-\log p(x_i|x_i;f^T,f^S)]$ when $\tau=1$. %
Since NCE allows us to fit unnormalized models, we adopt $Z_{0}$ estimated from the first training batch as a constant approximate divisor and use $\exp(f^T(x_i)^{\prime} f^S(x)/ \tau)/Z_{0}$ in place of $p(x|x_i;f^T,f^S)$ during training.

To learn $p_d(\cdot|x_i)=p(x|x_i;f^T,f^S)$, we build an auxiliary binary classifier between data and noise samples. Given a training sample $x_i$ for the teacher, we treat $x_i$ as a data sample for the student. The choice of the noise distribution is application specific; in this paper we use a uniform distribution over ${x_j}_{j\neq i}$ for the unsupervised case when we have no labels or ${x_j}_{y_j \neq y_i}$ for supervised case, where $y_i$ represents the label associated with sample $x_i$. The density of the noise distribution is $p_n(\cdot|x_i) = 1/n$, and we use $n=N$ as an approximation for simplicity. If we sample $k$ noise samples to pair with each data sample, the posterior that sample $x$ on the student side comes from the data distribution given $x_i$ from the teacher is:
\vspace{-10pt}
\begin{eqnarray}
    P(D=1|x;x_i) = \frac{p_d(x|x_i)}
    {p_d(x|x_i) + k p_n(x|x_i)}
    \label{eqn:posterior}
\end{eqnarray}
Therefore, we approximate the full softmax by training to minimize the negative log-posterior probability of label D over the data and noise samples:
\begin{eqnarray}
    \mathcal{L}_{contrast}^{NCE} = - \mathbb{E}_{x_i \sim p(x)}[
    \mathbb{E}_{p_d(\cdot | x_i)}[\log(P(D=1|x;x_i))] + k \mathbb{E}_{p_n(\cdot | x_i)}[\log(1-P(D=1|x;x_i))]
    ]
    \label{eqn:loss_NCE}
    \vspace{-10pt}
\end{eqnarray}

The above $p(x|x_i;f^T,f^S)$ treats the teacher as anchor, i.e., iterating over $j$ on the teacher side in the denominator of Eq.~\ref{eqn:prob}. Symmetrically, we can treat the student as anchor and iterate on the student side, which results in a similar NCE loss. During training, we add them up for completeness.




We adopt this approximate contrastive loss %
for knowledge distillation in $3$ scenarios: model compression, where the student network is a ``simpler" model than the teacher network; cross-modal transfer, where the student network is dedicated to a different task or dataset than the teacher network; and ensemble distillation, where the student compresses the information from multiple teacher networks into a single network. For all the methods, we apply the contrastive loss at the penultimate layer representation. The teacher networks are always fixed, and only the parameters of the student network are updated. In practice, since the dimensionality of teacher and student feature spaces may be different, we add a linear projection layer on the spaces to transform them into the same dimension so that the inner product in Eq.~\ref{eqn:prob} can be computed after we further normalize them by $\mathcal{L}$-2 norm. 

\textbf{Implementation.} In practice, a better softmax approximation by $\mathcal{L}_{contrast}^{NCE}$ in Eq.~\ref{eqn:loss_NCE} is learnt by using many negative samples (see Sec.~\ref{sec:parameters}). To avoid very large batch sizes, we consider memory bank  implementations introduced by previous methods~\cite{wu2018unsupervised}. We maintain a memory bank to store latent features for each data sample. During training, we can efficiently retrieve a large number of noise samples from the memory bank without recomputing their features. The memory bank is dynamically overwritten by newly computed features with a momentum of $0.5$.

\vspace{-5pt}

==> text/method_new1.tex <==
Contrastive learning has been successfully used for representation learning in different contexts \citep{oord2018representation, hjelm2018learning,sermanet2018time}. The key underlying idea is very general: learn a representation that is close in some metric space for ``positive'' pairs and push apart the representation between ``negative'' pairs. 
Fig. \ref{fig:methods_diagram} gives a visual explanation for how we structure the learning for the three tasks we consider: model compression, cross-modal transfer and ensemble distillation. 

\vspace{-5pt}
\subsection{Contrastive loss}
\vspace{-5pt}
We are given two deep neural networks, a teacher $f^T$ and a student $f^S$. Let $x$ be the network input; we denote representations at the penultimate layer (before logits) as $f^T(x)$ and $f^S(x)$ respectively. Let $x_i$ represent a training sample, and $x_j$ another randomly chosen sample. We would like to push closer the representations $f^S(x_i)$ and $f^T(x_i)$ while pushing apart $f^S(x_i)$ and $f^T(x_j)$. For ease of notation, we define random variables $S$ and $T$ for the student and teacher's representations of the data respectively:
\begin{align}
    x &\sim p_{\texttt{data}}(x) &&\triangleleft \quad \text{data}\\
    S &= f^S(x) &&\triangleleft \quad \text{student's representation}\\
    T &= f^T(x) &&\triangleleft \quad \text{teacher's representation}
\end{align}
Intuitively speaking, we will consider the joint distribution $p(S,T)$ and the product of marginal distributions $p(S)p(T)$, so that, by maximizing KL divergence between these distributions, we can maximize the \emph{mutual information} between student and teacher representations.
The true joint or product of marginals probability distributions are unknown; hence we must estimate them from samples that are drawn from the respective distributions, and assume some family of functions to parameterize the distributions, as is commonly done in related work such as \cite{oord2018representation, hjelm2018learning}.

To achieve this, we work with a family of unnormalized distributions $h$ i.e. functions that satisfy the following property: $h: \{\mathcal{T}, \mathcal{S}\} \rightarrow [0,1]$:
\begin{equation}
    h(T, S) = \frac{e^{T^{\prime}S/\tau}}{e^{T^{\prime}S/\tau} + M}
    \label{eqn:h}
\end{equation}
where $\tau \ll 1$ and $M < 1$ are hyperparameters. (see the appendix for an explanation of how we choose these parameters). Here $P_{TS} = e^{T^{\prime}S/\tau}$ represents the unnormalized probability of the joint or product of marginals, depending on whether the tuple $(T, S)$ is sampled from the joint distribution or product of marginals. The parameters of this family of functions are the parameters of the student network $S$.

Now, suppose in our data, we are given $1$ congruent pair (drawn from the joint distribution, i.e. the same input provided to $T$ and $S$) for every $N$ incongruent pairs (drawn from the product of marginals; independent randomly drawn inputs provided to $T$ and $S$). Then let us consider the loss function:
\begin{equation}
    \mathcal{L}_{contrast} = -\argmax_{h} \mathbb{E}_{T} \left[ ~\mathbb{E}_{S^+} \log h(T, S^+) + N~\mathbb{E}_{S^-} \log(1 - h(T, S^-)) \right]
    \label{eqn:loss_NCE}
\end{equation}
The first term in this loss corresponds to maximizing the (parameterized, unnormalized) $\log$-probability of samples $S^+$ drawn from the congruent samples (joint distribution); the second term corresponds to minimizing the $\log$-probability of samples $S^-$ drawn from the incongruent (product of marginal) distributions. Note that this loss function jointly optimizes the estimator (often called a critic) and the student network. 

Our loss function maximizes a lower bound to the mutual information between $T$ and $S$. A few simple manipulations show this connection:
\begin{eqnarray}
    -\mathcal{L}_{contrast} &=& \sum_T \left[ \sum_{S^+} \log \frac{P_{TS^+}}{P_{TS^+} + M} + N \sum_{S^-} \log \frac{M}{P_{TS^-} + M} \right] \label{eqn:term0} \\
    &=& \sum_T \left[ \sum_{S^+, S^-} \log \frac{P_{TS^+}}{P_{TS^+} + P_{TS^-}} +  \sum_{S^+, S^-} \log (P_{TS^+} + P_{TS^-}) \right] \label{eqn:term1} \\ &-& \sum_T \left[ \sum_{S^+} \log (P_{TS^+} + M) + N \sum_{S^+} \log (P_{TS^-} + M) -  N |\{S^-\}| \log M \right] \label{eqn:term2} \\
    & \leq & I(T; S) - \log N \label{eqn:term3} \\ 
    &+& \sum_T \sum_{S^+, S^-} \log \frac{P_{TS^+} + P_{TS^-}}{(P^{TS^+} + M)(P^{TS^-} + M)} \label{eqn:term4} \\ 
    &-& (N - 1) \sum_T \sum_{S^-} \log (P_{TS^-} + M) + N |\{S^-\}| \log M \label{eqn:term5} \\
    & \leq & I(T; S) \label{eqn:term6}
\end{eqnarray}

where $I(T; S)$ is the mutual information between the distributions of teacher and student embeddings. \eqref{eqn:term1} and \eqref{eqn:term2} follow from \eqref{eqn:term0} with a simple re-arrangement. \eqref{eqn:term3} follows from the first term in \eqref{eqn:term1} using the same derivation as InfoNCE \cite{oord2018representation}. Since we use small temperatures $\tau$, the unnormalized probabilities $P_{TS^+}$ and $P_{TS^-}$ are always greater than $1$, so that \eqref{eqn:term4} is less than $0$. For the same reason, the first term in \eqref{eqn:term5} is negative. Finally, since $M < 1$, the second term in \eqref{eqn:term5} is also negative. From all these considerations, the final inequality \eqref{eqn:term6} follows; thus the negative of our loss function is a lower bound to the mutual information, and so minimizing our loss Eq. \eqref{eqn:loss_NCE} corresponds to increasing this lower bound.

Our loss functions combines ideas from both InfoNCE \cite{oord2018representation} and NCE \cite{gutmann2010noise}. We use the idea of contrastive a single positive and multiple negatives, that was used in InfoNCE. But instead of directly using the InfoNCE formulation, we use an NCE-like loss similar to that proposed in \cite{mnih2013learning}. In our case, the noise distribution of NCE is a uniform distribution whose purpose is to approximate the intractable full softmax distribution over all samples (tuples $(T, S)$. Finally, we note that NCE as originally proposed in \cite{gutmann2010noise} does not have any connection to mutual information maximization, unlike our proposed loss.


==> text/method_other_objectives.tex <==
\subsection{Other knowledge distillation objectives}

\vspace{-5pt}

Several distillation objectives, such as KL divergence and attention transfer, have been proposed to transfer knowledge from a large pre-trained teacher network to a smaller student. 


\textbf{Knowledge Distillation (KD)} The knowledge distillation loss was proposed in~\cite{hinton2015distilling}. In addition to the regular cross-entropy loss between the student output $y^S$ and one-hot label $y$, it asks the student network output to be as similar as possible to the teacher output by minimizing the cross-entropy between their output probabilities. The complete objective is:
\vspace{-2pt}
\begin{equation}
    \mathcal{L}_{KD} = (1-\alpha) H(y, y^S) + \alpha \rho^2 H(\sigma(z^T/\rho), \sigma(z^S/\rho))
    \label{eqn:kd}
\end{equation}
where $\rho$ is the temperature, $\alpha$ is a balancing weight, $\sigma$ is softmax function. 


\textbf{Attention Transfer (AT)} Matching the attention maps between the teacher and student is another way to transfer knowledge~\cite{zagoruyko2016paying}. The student is trained by minimizing:
\vspace{-2pt}
\begin{equation}
    \mathcal{L}_{AT} = H(y, y^S) + \beta \sum_{i=1}^{L}
    \left\Vert \frac{A_i^T}{\| A_i^T \|_2} - \frac{A_i^S}{\| A_i^S \|_2} \right\Vert_2
    \label{eqn:at}
\end{equation}
where $\beta$ is a weight parameter, $A_i^T$ and $A_i^S$ represent the $i$-th attention map in teacher and student networks. An assumption made in AT is that there are such layers in student and teacher network which can be directly compared using an $L_2$ regression loss.  

\textbf{Regression (FitNet)} Matching teacher features by regressing student features is first used in~\cite{ba2014deep} and further demonstrated by~\cite{romero2014fitnets}. The objective is:
\vspace{-2pt}
\begin{equation}
    \mathcal{L}_{FitNet} = H(y, y^S) + \beta / 2 
    \left\Vert f_i^T - r(f_j^S; W) \right\Vert_2
    \label{eqn:fitnet}
\end{equation}
where $f_i^T$ and $f_j^S$ are features at $i$-th and $j$-th layer from the teacher and student network respectively. $r(\cdot;W)$ is the regression function parameterized by $W$. 

\textbf{Contrastive Knowledge Distillation (CRD)} Our CRD objective aims at distilling structured knowledge from the teacher representations. The objective we minimize is thus:
\vspace{-2pt}
\begin{equation}
    \mathcal{L}_{CRD} = H(y, y^S) + \beta \mathcal{L}_{contrast}(T, S)
    \label{eqn:ckd}
\end{equation}
where $\beta$ is a hyperparameter and we find that $\beta \in [0.2, 3.0]$ produces good results. In this paper, we fix $\beta=0.8$ for all our experiments.

\vspace{-5pt}





